RLER-TTE: An Efficient and Effective Framework for En Route Travel Time Estimation with Reinforcement Learning

En Route Travel Time Estimation (ER-TTE) aims to learn driving patterns from traveled routes to achieve rapid and accurate real-time predictions. However, existing methods ignore the complexity and dynamism of real-world traffic systems, resulting in significant gaps in efficiency and accuracy in real-time scenarios. Addressing this issue is a critical yet challenging task. This paper proposes a novel framework that redefines the implementation path of ER-TTE to achieve highly efficient and effective predictions. Firstly, we introduce a novel pipeline consisting of a Decision Maker and a Predictor to rectify the inefficient prediction strategies of current methods. The Decision Maker performs efficient real-time decisions to determine whether the high-complexity prediction model in the Predictor needs to be invoked, and the Predictor recalculates the travel time or infers from historical prediction results based on these decisions. Next, to tackle the dynamic and uncertain real-time scenarios, we model the online decision-making problem as a Markov decision process and design an intelligent agent based on reinforcement learning for autonomous decision-making. Moreover, to fully exploit the spatio-temporal correlation between online data and offline data, we meticulously design feature representation and encoding techniques based on the attention mechanism. Finally, to improve the flawed training and evaluation strategies of existing methods, we propose an end-to-end training and evaluation approach, incorporating curriculum learning strategies to manage spatio-temporal data for more advanced training algorithms. Extensive evaluations on three real-world datasets confirm that our method significantly outperforms state-of-the-art solutions in both accuracy and efficiency.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> revision/meta.tex <==
\section{Meta-Reviewer}


% \section*{Comments from Meta-Reviewer and Shepherd}

% \begin{enumerate}
% [leftmargin=*,itemindent=0.6cm]

    \noindent
    % \item[\textbf{M1.}] 
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{Required Changes 1.}
    Assess alternative reinforcement learning strategies, or better justify why DDQN is the only strategy needed. Further, describe how the hyperparameters for DDQN were set. [R1.O1]
    \end{tcolorbox}

    \begin{response}[\textbf{MR.1}]
        Thanks for your valuable suggestions. We have included two additional reinforcement learning methods, PPO~\cite{PPO} and A3C~\cite{A3C}, in the experimental section. The corresponding experimental results are presented in Table 3 and Table 4, with a detailed analysis provided in Sections 6.4 and 6.6. Moreover, detailed descriptions of the hyperparameters for Double DQN have been added in Section 6.1 under the \textbf{Experimental Settings}.
    \end{response}
    
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{Required Changes 2.}
    An additional experiment varying the time interval of the requests, since this parameter balances efficiency and accuracy between offline and en route predictions. [R1.O2]
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{MR.2}]
        Thanks for your valuable suggestions. We have added Section 6.5 to present the impact of varying the time interval \( t \) between prediction requests on the experimental results. Since this hyperparameter is unique to the ER-TTE method, we compared \textbf{\modelName} with the state-of-the-art method \textbf{MetaER-TTE} under time intervals ranging from 15 seconds to 180 seconds. In real-world application scenarios of the ER-TTE task, the interval between prediction requests should not be excessively long. A long interval would result in almost no en-route prediction requests. For example, the average travel times of the \textit{Chengdu} and \textit{Porto} datasets are 500.65s and 479.12s, respectively. If we set the interval to 5 or 10 minutes, most trajectories would have only one or two, or even no, en-route prediction requests, which is inconsistent with the application scenario of ER-TTE techniques. Moreover, as the time interval increases, the overall system performance deteriorates, indicating that a long interval is not a reasonable design choice. The experimental results are presented in Figure 7, with a detailed discussion and analysis provided in Section 6.5.


        % This will help us verify the robustness of our method and analyze whether our framework performs effectively across various \( t \) values or if there are certain limitations under specific conditions.
    \end{response}

    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{Required Changes 3.}
    \textit{Articulate the differences between this paper and~\cite{RTTE}. [R2.O6]}
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{MR.3}]
        Thanks for your valuable suggestions. In \textbf{Offline Travel Time Estimation} (Section 7.1),we provided a more detailed explanation of the offline TTE methods, including that of~\cite{RTTE}, and conducted an in-depth analysis of their shortcomings. Additionally, we elaborate on the differences between~\cite{RTTE} and our proposed approach in terms of application scenarios, data processing, and the overall framework. Furthermore, in \textbf{Online Travel Time Estimation}, we have highlighted our scientific contributions from an online perspective, including the introduction of a novel real-time framework and a curriculum learning component for managing training data. The online challenges addressed in this work are fundamentally different from the issues focused on in~\cite{RTTE}.
        
        % The application scenario of our work is fundamentally different from that of~\cite{RTTE}. First, our task focuses on online ER-TTE, whereas the task in~\cite{RTTE} is an offline TTE task. Our work emphasizes the integration of real-time data into a novel framework that balances efficiency and performance in a complex and dynamic online system. In contrast, ~\cite{RTTE} focuses more on static trajectory data to provide accurate predictions, placing a greater emphasis on technical accuracy and the spatio-temporal characteristics of the data, which is only somewhat similar to the Predictor task in our framework.
        
        % Secondly, the dynamic data in our work is real-time data collected from the journey just taken by the user in an online scenario. In~\cite{RTTE}, however, the so-called dynamic data is simulated under different traffic conditions. Essentially, it remains a static characteristic of the road network. From a data perspective, our work focuses on the characteristics of real-time data, such as driving behavior. However, characteristics like heterogeneity and proximity in~\cite{RTTE} pertain to the internal features of static data, which are not the primary focus of our work involving real-time data.
        
        % Finally, our framework is specifically designed for the unique scenario of the ER-TTE task. From a framework perspective, we address a completely different problem than~\cite{RTTE}. We have designed a framework composed of a lightweight Decision Maker and a complex Predictor. Additionally, we have carefully designed a curriculum learning strategy to manage training data, addressing the data explosion issue inherent in the ER-TTE scenario. 
        
        % In the related work section, we will expand our discussion of~\cite{RTTE} to help readers better understand the differences between our work and~\cite{RTTE}.
    \end{response}

    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{Required Changes 4.}
    Describe the difficulty measurement model in more detail, and provide more experimental evidence of its efficacy: How do we know it works well, and undershot circumstances does it work poorly? How do the choices of hyperparameters affect the results (partitioning of the trajectory, N, the number of metasets)? [R2.O7]
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{MR.4}]

        Thanks for your valuable suggestions. In Section 5, we provide a more detailed explanation of the two key components of curriculum learning: the trajectory difficulty measurer and the training scheduler. Figure 4 has been revised to include more details, and additional descriptions have been provided accordingly. We have also enhanced the discussion on the difficulty score and added Algorithm 2 to illustrate the scheduling strategy of curriculum learning. In Section 6.2, we conducted comprehensive experiments on curriculum learning-related hyperparameters, such as parameters related to curriculum partitioning, and provided a detailed presentation of the performance of curriculum learning under different settings.
        
        % Thanks for your valuable suggestions. We will provide a more detailed explanation of the curriculum learning component, including a thorough description of the intricately designed trajectory difficulty measurer and the training scheduler, elaborating on the working principles and internal mechanisms of each component. Additionally, we will include more experiments related to curriculum learning to further demonstrate the effectiveness of our approach and explore its limitations. We will discuss in detail the robustness and limitations of the evaluation scores produced by the difficulty measurer. In the experimental setup, we will conduct additional experiments by treating trajectory length segmentation, the number of meta-sets, and \(N\) as hyperparameters to comprehensively assess the impact of curriculum learning. Special attention will be given to the relationship between the number of meta-sets and the difficulty scores, exploring whether the scoring system can maintain its discriminative capability as the number of meta-sets increases.
    \end{response}

    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{Required Changes 5.}
    Add more discussion of related work on this topic, including~\cite{latte, vldb20, HRA, SSML}.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{MR.5}]
        Thanks for your valuable suggestions. In Section 7, we further expanded the discussion on related work in the data management community concerning the topic of this paper. We introduced these works from the perspectives of spatio-temporal data management and data processing, highlighting the differences between them and our proposed approach.
    \end{response}

    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{Required Changes 6.}
    See reviews for various presentation issues. [R1.O5, R2.M1, R3.O1]
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{MR.6}]
         We appreciate the reviewer’s thorough examination of our work. We have addressed all presentation issues mentioned in the reviews and ensured that the formatting and layout adhere to the appropriate standards.
    \end{response}


% \end{enumerate}


==> revision/reviewer1.tex <==
\section{Reviewer 1}

% \begin{enumerate}[leftmargin=*,itemindent=0.6cm]

    
    % \item[\textbf{O1.}] 
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O1.}
    The paper proposes a framework that includes a decision maker in addition to a predictor. Although this work introduces the concept of the decision maker, it is formulated using a Markov decision process and implemented with the existing Double Deep Q-Network (Double DQN). In the experiments, the authors only compare their selection of Double DQN with a transformer model. To justify the selection of Double DQN, it should also be compared with alternative reinforcement learning methods. Additionally, there is no mention or experimentation regarding the selection of hyperparameters related to reinforcement learning.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R1.O1}]
        % Thank you for your insightful feedback. In response to your comments, we will design additional experiments to study alternative reinforcement learning methods and provide a detailed explanation of the settings of hyperparameters related to reinforcement learning, as elaborated in our response to MR.1.
        Please refer to MR.1
    \end{response}

    
    % \item[\textbf{O2.}] 
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O2.}
    The paper does not show a comparative analysis with baselines by varying the time interval of requests. For example, if requests for re-estimation of travel time arrive at intervals of t minutes, then t can be varied as 5, 10, or 15 minutes.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R1.O2}]
        % Thanks for your valuable suggestions. We agree that the interval \( t \) between prediction requests is indeed an important hyperparameter. Therefore, we have conducted additional experiments to study the impact of different values of \( t \) on our method and the SOTA method, as explained in our response to MR.2.
        Please refer to MR.2.
    \end{response}

    % \item[\textbf{O3.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O3.}
    The quality of writing in the paper needs improvement. The technical content is hard to read. For instance, the paper does not adequately explain or introduce the symbols used in the algorithms and functions. The experimental results are also not well explained.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R1.O3}] \label{res_r1_o3}
        Thanks for your valuable suggestions. We have improved the overall writing quality of the paper and revised the technical content. In Algorithm 1, we removed the previously redundant symbols, updated the algorithmic content, and ensured that the role of all existing symbols is clearly explained. In the experimental section, we added a substantial number of experiments and provided detailed analysis and interpretation of the results.
    \end{response}
    
    % \item[\textbf{O4.}] 
    
    \noindent  
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O4.}
    It is not clear why the complexity of the proposed framework is better than existing solutions, as presented in Table 1. The proposed framework includes both a decision maker and a predictor, whereas previous solutions only include a predictor. Furthermore, the predictor in the proposed framework is implemented using existing solutions.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R1.O4}]
        Thanks for your valuable suggestions. In \textbf{Complexity Analysis} of Section 4.3, we provided a clearer explanation, emphasizing that this section compares the Decision Maker in RLER-TTE with the baseline methods and clarifies the rationale behind this comparison. Additionally, we revised Table 1 to eliminate any previously unclear expressions.
    \end{response}

    % \item[\textbf{O5.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O5.}
    The caption of Figure 1 is incorrect, and Figure 1 needs to be explained in the Introduction section. Figures 7, 8, and 9 are not readable.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R1.O5}]
        Thanks for your valuable suggestions. We revised the caption of Figure 1 and provided a detailed explanation of it in Section 1. For the original Figure 7, we converted it into Table 5 in Section 6.7, following the format of ~\cite{ODT}, to more intuitively present the scalability experimental results. Regarding Figures 8 and 9, which are typical example plots in TTE studies, we revised the explanations in Section 6.8 to clarify the purpose of these two figures, ensuring that readers can easily understand them.
    \end{response}

% \end{enumerate}

==> revision/reviewer2.tex <==
\section{Reviewer 2}

% \begin{enumerate}[leftmargin=*,itemindent=0.6cm]

    % 
    % \item[\textbf{O1.}]
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O1.}
    SIGMOD is the wrong outlet for this type of paper. An ML outlet is a much better fit for the paper. The paper stitches together a framework of many different components but none of the components is described in detail. Especially the data management parts, the data processing parts, and the data structures are not described in detail. This also show in the baselines that the authors use to compare their work to. These are DeepTTE (AAAI), STANN (IEEE Access), ConST (SIGKDD), SSML (SIGKDD), MetaER-TTE (IJCAI), MAML (ICML). Clearly these are not database system venues. A paper that uses as baselines only works published in a different community should motivate why this makes sense and identify the findings that are relevant to the data management community.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O1}]

    \iffalse
        We believe that our work is a good fit for SIGMOD, as there are important precedents published at related field conferences, such as~\cite{odtto, sigmod07, vldb20, RTTE}. These works, like ours, apply advanced ML techniques to the processing and optimization of spatio-temporal data. This demonstrates that using ML techniques to solve data-intensive problems is an accepted research path within the database community. Our work continues this tradition but introduces new contributions in system design and data management.
        \fi

        We believe our work is well-suited for SIGMOD. Firstly, several prior studies that apply machine learning techniques to process or predict spatio-temporal data, such as~\cite{odtto, sigmod07, vldb20, RTTE}, have been published at conferences in related fields. This indicates that using machine learning to address data-intensive problems is an accepted research direction within the database community. Secondly, our work focuses on optimizing both the efficiency and accuracy of the ER-TTE task, rather than concentrating on optimizing the estimation model. Actually, TTE work published in the ML domain typically focuses more on travel time estimation model design and optimization, and these models serve as a component within our broader framework. Therefore, our work differs fundamentally from papers published in ML-focused conferences. In summary, the system framework we designed dynamically adjusts data streams, optimizing the entire data processing pipeline for ER-TTE tasks. Beyond the core framework, we also designed a curriculum learning strategy to manage massive spatio-temporal data in the model training process.
        
        We have enhanced the discussion of data management, data processing, and data structure aspects in our paper. In both Section 1 and Section 7, we have emphasized the scientific contributions of our work to the field of data management. Additionally, we have enriched the details related to data management in Section 5, particularly by refining key components of curriculum learning. We have made further modifications throughout the paper to ensure that it contributes to meaningful technical advancements for the community.
    \end{response}

    % \item[\textbf{O2.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O2.}
    The scientific novelty must be spelled out much more crisply. For instance how does the paper advance the state of the art of reinforcement learning? Using a reinforcement learning component make sense from an engineering perspective but does not make this a scientific contribution. The same observation applies to the separation of features into, respectively, online and offline features. This seems a reasonable implementation. What are the generally valid research insights for readers? The main scientific contribution of the paper must be pinpointed precisely. If reinforcement learning is not a contribution then the paper must be re-focused on the scientific contribution of this submission.
    \end{tcolorbox}
    
    \begin{response}[\textbf{R2.O2}]

    \iffalse
        Our primary scientific contribution lies in proposing and validating a real-time data processing framework suitable for online scenarios. This framework resolves the conflict between efficient data processing and model invocation optimization in online real-time systems by redefining the data processing pipeline. During the design of this framework, we encountered numerous scientific challenges, each of which we addressed with corresponding solutions. Our research is not merely an engineering integration of existing technologies; instead, we propose a novel data processing pipeline that offers a new approach to tackling complex ER-TTE tasks, significantly enhancing overall system efficiency and performance. These methods and strategies can be broadly applied to other similar online real-time data processing systems, making this work of general research significance.
    \fi
        
        In Section 1, We have restated and elaborated on the scientific contributions of this paper. Our primary contribution lies in proposing and validating an efficient and effective framework suitable for the ER-TTE task, which, to the best of our knowledge, is the first of its kind. This framework addresses the trade-off between reusing previous results and employing effective models to handle large-scale ER-TTE requests efficiently.
        
        To overcome the challenges introduced by the framework, we model the online decision-making process as a Markov Decision Process and carefully design states that sufficiently represent the characteristics of the data, along with a well-defined reward function. Similar to many ML4DB tasks, our use of reinforcement learning with carefully designed feature representation and encoding serves as an essential tool to address the data management challenges within the framework.
        
        Our research is not merely an engineering integration of existing technologies. Rather, we introduce a novel pipeline that provides a new approach for tackling complex ER-TTE tasks, significantly improving overall system efficiency and performance. Furthermore, the proposed methods and strategies can be generalized to other real-time decision-making systems, underscoring the broad research significance of this work.
        
        Finally, we further highlight the training and evaluation standards we established for ER-TTE system and elaborate on the scientific contributions of curriculum learning from a data management perspective.
        
        
    \iffalse
        Our primary scientific contribution lies in proposing and validating an efficient and effective framework suitable for the ER-TTE task. The framework resolves the tradeoff between reusing results and invoking effective models when handling large-scale ER-TTE requests. During the design of this framework, we encountered numerous challenges, each of which we addressed with ML-related solutions. This approach is similar to many studies in ML4DB tasks, where advanced ML models are applied to address data management challenges. 
        Therefore, our research is not merely an engineering integration of existing technologies; instead, we propose a novel pipeline that offers a new approach to tackling complex ER-TTE tasks, significantly enhancing overall system efficiency and performance. These methods and strategies can be broadly applied to other similar real-time decision systems, making this work of general research significance.
        
        Innovations in the ML field tend to focus more on prediction model optimizations. 
        % When it comes to addressing efficiency issues, the ML field typically leans towards designing smaller models. 
        In contrast, our work aims to address efficiency issues from a data processing perspective, creatively proposing a novel pipeline for ER-TTE. Moreover, with our novel framework, the ML field can concentrate on developing more powerful Predictor models, as our framework significantly reduces the overhead of such models and provides the potential for jointly training new models that better align with the ER-TTE pipeline we have defined. 
        % A more powerful model might mean fewer model invocations.
        
        ML techniques like reinforcement learning are primarily tools for implementing the framework, with the core purpose of optimizing the invocation of complex deep learning models within the framework, as they can adaptively make decisions in dynamic and uncertain online environments. This paper demonstrates how machine learning techniques can be innovatively applied to online data processing systems, opening new avenues for research in the fields of databases and information systems.
        
        We will also revise the description of our scientific contributions related to ML techniques in the paper to clearly reflect their role and impact within our framework.
    \fi
    \end{response}
    
    % \item[\textbf{O3.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O3.}
    The sketching of the state information in Section 3 is good and should be extended to precisely define and illustrate feature vectors. The more and less important information of your state should be identified.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O3}]
        % \redcolor{TODO}
        Thank you for your valuable suggestions. First, we have further refined the state information in Section 3 and provided a detailed definition of each feature. Second, in Section 4.1, we have elaborated on the data characteristics included in the state, analyzing the role of different online and offline features in various components of the framework. Moreover, we have highlighted the more significant features within the state.
    \end{response}

    % \item[\textbf{O4.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O4.}
    The use of user names in the source code violates the anonymity requirements of SIGMOD.
    % An example is the user name haitao in "/home/haitao/data/zigzag_zoom_hash/MetaER-TTE".}
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O4}]
        % \redcolor{TODO}
        The project configuration file contained a path with a word resembling a username, which did not correspond to a real full name, making it highly unlikely to reveal the authors' identities. However, to eliminate any potential concerns, we have revised the path to remove any ambiguity. We are committed to adhering to the anonymity guidelines and can confirm that the current source code fully complies with these rules.
        \iffalse
        Thank you for your valuable suggestion. There was a path in the ".idea" project configuration file that included a partial username, which does not appear to correspond to a real author name. We believe this does not compromise author anonymity. However, to prevent any misunderstanding, we have revised the path. We are committed to following the anonymity guidelines, and we confirm that the current source code fully complies with these rules.
        \fi
    \end{response}

    % \item[\textbf{O5.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O5.}
    The paper does not provide any guarantees and properties. It is important for a research paper to reflect about and add results about limitations, guarantees, etc. As is the paper offers a carefully done description of an extensive PyTorch implementation. What are the scientific learnings and generally valid insights for readers?
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O5}]
        Thanks for your valuable suggestions. We have rigorously rearticulated the scientific contributions of this paper to ensure that our work provides valuable insights to the data management community. Our approach provides a novel solution for real-time data processing, demonstrating how to reduce system burdens through model invocation optimization. Moreover, we have enhanced the paper with extensive experiments to explore the limitations of our approach. The experiments in Section 6.5 thoroughly illustrate the framework’s performance under various design configurations, clarifying the scope and potential boundaries of the current method.
        
    \iffalse
        Thanks for your valuable suggestions. We will add content to discuss the limitations of our work. In particular, we will clarify the scope and potential boundaries of the current approach and explore directions for future improvements. 
        % Additionally, we will conduct a deeper analysis of our experimental results to offer useful and broadly applicable scientific insights to the readers.

        Through the in-depth analysis of our experimental results, we will distill broader scientific insights, such as how to effectively manage large-scale spatio-temporal data in real-time data streams and how to reduce system burdens through model invocation optimization. Our work has broad practical value in data management, as our innovative pipeline design showcases how intelligent data stream management and system resource allocation can optimize the efficiency of complex real-time tasks. With these scientific contributions, the data management community can gain new technical tools to tackle more challenges in designing online data processing systems in the future.
        
        % We recognize the importance of discussing the limitations of the research and providing certain assurances in an academic paper. This helps readers better understand the scope and potential constraints of the study.

        % Following the reviewer's suggestion, we will add content to discuss the limitations of our work and any possible assurances. In this section, we will clarify the scope and potential boundaries of the current approach and explore directions for future improvements. Additionally, we will conduct a deeper analysis of our research findings to offer useful and broadly applicable scientific insights to the readers.
    \fi
    \end{response}
    

    % \item[\textbf{O6.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O6.}
    In terms of related work a more careful detailing of the difference to~\cite{RTTE} is necessary. The authors briefly mention that~\cite{RTTE} consider spatio-temporal features such as heterogeneity and proximity. This is not detailed enough. Your state also includes spatio-temporal features. Do you consider heterogeneity and proximity? Why/why not? The difference between the architecture and processing pipeline in~\cite{RTTE} and your framework must be worked out in detail. Many elements are quite similar, which limits the novelty of the proposed framework.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O6}]
        % Thanks for your valuable suggestions. We have provided a detailed response in our response to MR.3. Our framework addresses a completely different task scenario compared to the framework in~\cite{RTTE}. And our work specifically focuses on real-time data, which is not present in~\cite{RTTE}. We will expand the discussion in the related work section to clearly describe these differences, helping readers better understand the novel approach we propose.
        Please refer to MR.3.
    \end{response}

    % \item[\textbf{O7.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O7.}
    The trajectory difficulty measurer and the training scheduler in Section 5 are interesting ideas. Again it is essential to advance these ideas to results (a couple of paragraphs per component is not sufficient to work out crisp research results). Algorithms, properties, evaluations are missing. In addition to the high level illustration in Figure 4 the authors could set up a running example with a few example trajectories and use it to illustrate, e.g., the difficulty score computation. How good and robust is the proposed difficulty score? What are its limitations and when does it not work well? How does the partitioning of the route length affect the difficulty score? How do you choose N? How do you choose the number of metasets? How is the number of metasets related to the quality of the difficulty score?
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O7}]
        % Thanks for your valuable suggestions. We appreciate your concern regarding the curriculum learning component, and we have provided a detailed response in MR.4. We will further enhance the explanation of the curriculum learning section, including the key components and the difficulty measurement scores. Additionally, we will conduct supplementary experiments to further validate the hyperparameters related to curriculum learning.
        Please refer to MR.4.
    \end{response}

    % \item[\textbf{O8.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O8.}
    At the beginning of Section 5 the authors write "As we proposed an end-to-end training method, the number of samples generated from each trajectory increased exponentially." Please add a proof that the end-to-end training method leads of the exponential growth of the number of samples. This finding must also be connected to the complexity analysis and the experimental result. In these no exponential growth can be found. Please work out in detail how you got rid of the exponential growth.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O8}]
        % \redcolor{TODO}
        Thank you for your valuable suggestions. We apologize for the unclear description at the beginning of Section 5, which caused some ambiguity. The intended meaning was that the data volume increased significantly. For example, if the average trajectory length is 30, the data volume increases 30-fold, as each of the 30 trajectory links represents a new online state with different traveled segments, resulting in 30 distinct training data points. To address this, we designed a curriculum learning mechanism to improve training efficiency under such data volume, which has been proven effective in our experimental results.
        We have revised the original wording and provided a more detailed explanation in Section 5.
    \end{response}

    % \item[\textbf{O9.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O9.}
    It is important to work out the limitations as well. What are the cases when RLER-TTE does not perform well? It is not very plausible that a method beats the time/space tradeoff and is better than all other methods in all settings.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O9}]
        % \redcolor{TODO}
        Thank you for your valuable suggestions. In Section 6, we have added a substantial number of experiments, including new datasets and additional time interval experiments, to explore the limitations of our framework. In Section 6.5, we present the performance of our method compared to state-of-the-art method under different time intervals. Due to our innovative framework, our method shows a clear advantage in terms of efficiency. However, as the interval increases, the improvements in performance gradually diminish, which we have analyzed in detail in Section 6.5.
    \end{response}

    % \item[\textbf{O10.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O10.}
    The authors should experiment with datasets that have been used in related works to facilitate comparison and helps readers to better appreciate your contribution. For instance~\cite{ODT} uses the real-world taxi trajectory datasets collected from Chengdu for estimating the travel time in their experiments. Instead of using a different Chengdu dataset the authors should use the same dataset so that it becomes possible to relate the two approaches for travel time estimation.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O10}]
        % Thanks for your valuable suggestions. The work~\cite{odtto} did not open source their code and dataset, but our data is from the same source as the data used in~\cite{odtto}, both collected from Didi Chuxing's Chengdu taxi data. While we did not use the exact same dataset, the data source and collection methods are identical. We will further elaborate on the relevance of our work to~\cite{odtto} in the related work section.
        Thanks for your valuable suggestions. The work~\cite{ODT} did not open source their code and dataset, but our data is from the same source as the data used in~\cite{ODT}, both collected from Didi Chuxing's Chengdu taxi data. Additionally, the task in~\cite{ODT} is OD-based TTE, whereas our task is path-based TTE. All baseline methods have been tested on our dataset, and we will open-source our dataset once this paper is accepted. To strengthen the connection between our work and related research, we have additionally incorporated the \textit{Porto} dataset, which is the same dataset used by the state-of-the-art method~\cite{MetaER-TTE}, and has been widely studied in the spatio-temporal data domain~\cite{porto21, porto22}. In Section 7, we have made significant revisions to strengthen the connection and distinction between our work and related research, thereby highlighting the scientific contributions of our work.
    \end{response}

    % \item[\textbf{O10.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O11.}
    In the efficiency experiments it would be interesting to also add experiments with NU, ND and NA (as done for the effectiveness experiments).
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.O11}]
        % \redcolor{TODO}
        Thanks for your valuable suggestions. In Section 6.6, we present the efficiency results of the ablation experiments for NU, ND, and NA. Additionally, we have conducted a thorough investigation of the efficiency of the newly introduced ablation variants, \modelName-p and \modelName-a, and provided a detailed analysis of the results.
    \end{response}

    % \item[\textbf{M1.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{M1.}
    In figure 7 the units for the y-axis must be added.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.M1}]
        Thank you for pointing that out. Following the format of ~\cite{ODT}, we have reformatted the original Figure 7 into Table 5 to present the experimental results more intuitively and to ensure that the paper does not encounter any presentation issues.

 
    \end{response}

        % \item[\textbf{M2.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{M2.}
    Similar to RLER-TTE* (which uses SSML as a predictor) it would be interesting to see the runtime performance of RLER-TTE without the inference memory to understand the benefits of this component.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R2.M2}]
        Thanks for your valuable suggestions. However, the inference memory is a crucial component of our framework. It provides prediction results without invoking the Predictor, and removing it would fundamentally disrupt the framework’s operation. Therefore, it is not feasible to evaluate RLER-TTE without this component.
    \end{response}

    
% \end{enumerate}


% Innovations in the ML field tend to focus more on algorithmic and model optimizations. When it comes to addressing efficiency issues in real-time systems, the ML perspective often involves optimizing model design to reduce model size while ensuring higher accuracy. In contrast, our work approaches the problem from a data processing perspective, creatively proposing a novel pipeline for ER-TTE that redefines the data processing workflow. Our framework is better suited to the data management community, rather than being an innovation in ML technology. Moreover, with our novel framework, the ML field can focus on developing more powerful Predictor models, as our framework significantly reduces the overhead of such models and provides the potential for jointly training new models that better align with the ER-TTE pipeline we defined. A more powerful model might mean fewer model invocations.

% ML techniques like reinforcement learning are primarily tools for implementing the framework, with the core purpose of optimizing the invocation of complex deep learning models within the framework. We chose reinforcement learning agents not just to meet technical requirements, but because they can adaptively make decisions in dynamic and uncertain online environments—something that existing technologies cannot offer. By introducing reinforcement learning agents, we effectively reduced the number of model invocations while maintaining system prediction accuracy. This contribution demonstrates how ML technologies can be innovatively applied within data management systems, opening up new directions for research in the database and information systems fields.

% Our work provides the database and data management community with new perspectives and tools, particularly in handling real-time data and optimizing complex model invocations. Through the innovative pipeline design, we not only improved system efficiency but also paved the way for the application of more complex and powerful predictive models in the future. The breakthrough contributions of our framework in data management and system design prove that scientific innovation is not limited to algorithmic improvements but also includes how to efficiently integrate and apply these technologies to solve real-world engineering and scientific problems.

==> revision/reviewer3.tex <==
\section{Reviewer 3}


% \begin{enumerate}
% [leftmargin=*,itemindent=0.6cm]
% [rightmargin=*,itemindent=0.6cm]
% [leftmargin=*]

    % 
    % \item[\textbf{O1.}] 
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O1.}
    Several experimental figures have no labels on the axes, making it difficult to read efficiently.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R3.O1}]
        Thanks for your valuable suggestions. We have ensured that all figures in the paper have properly labeled axes, and we have reviewed all figures to guarantee their readability.
    \end{response}

    % \item[\textbf{O2.}]
    
    \noindent
    \begin{tcolorbox}[breakable, boxrule=0.5pt, 
    % colback=white,
    arc=3pt, outer arc=3pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
    \textbf{O2.}
    The related work section should explicitly distinguish the proposed work from the existing techniques.
    \end{tcolorbox}
    
    
    \begin{response}[\textbf{R3.O2}]
        Thanks for your valuable suggestions. In Section 7, we have made significant revisions to the related work to ensure a clear explanation. In Section 7.1, under \textbf{Offline Travel Time Estimation} and \textbf{Online Travel Time Estimation}, we have thoroughly articulated the differences between our work and existing approaches, while highlighting the scientific contributions of our work.

    \end{response}

% \end{enumerate}
